Miniaturized Microwave Devices and Antennas for Wearable, Implantable and Wireless Applications

This thesis presents a number of microwave devices and antennas that maintain high operational efficiency and are compact in size at the same time. One goal of this thesis is to address several miniaturization challenges of antennas and microwave components by using the theoretical principles of metamaterials, Metasurface coupling resonators and stacked radiators, in combination with the elementary antenna and transmission line theory. While innovating novel solutions, standards and specifications of next generation wireless and bio-medical applications were considered to ensure advancement in the respective scientific fields. Compact reconfigurable phase-shifter and a microwave cross-over based on negative-refractive-index transmission-line (NRI-TL) materialist unit cells is presented. A Metasurface based wearable sensor architecture is proposed, containing an electromagnetic band-gap (EBG) structure backed monopole antenna for off-body communication and a fork shaped antenna for efficient radiation towards the human body. A fully parametrized solution for an implantable antenna is proposed using metallic coated stacked substrate layers. Challenges and possible solutions for off-body, on-body, through-body and across-body communication have been investigated with an aid of computationally extensive simulations and experimental verification. Next, miniaturization and implementation of a UWB antenna along with an analytical model to predict the resonance is presented. Lastly, several miniaturized rectifiers designed specifically for efficient wireless power transfer are proposed, experimentally verified, and discussed. The study answered several research questions of applied electromagnetic in the field of bio-medicine and wireless communication.

==> MacroFile1.tex <==
\newcommand{\PdfPsText}[2]{
  \ifpdf
     #1
  \else
     #2
  \fi
}

\newcommand{\IncludeGraphicsH}[3]{
  \PdfPsText{\includegraphics[height=#2]{#1}}{\includegraphics[bb = #3, height=#2]{#1}}
}

\newcommand{\IncludeGraphicsW}[3]{
  \PdfPsText{\includegraphics[width=#2]{#1}}{\includegraphics[bb = #3, width=#2]{#1}}
}

\newcommand{\InsertFig}[3]{
  \begin{figure}[!htbp]
    \begin{center}
      \leavevmode
      #1
      \caption{#2}
      \label{#3}
    \end{center}
  \end{figure}
}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/Documents/LaTeX/CUEDThesisPSnPDF/thesis"
%%% End: 

